An Ultrahigh-energy $\gamma$-ray Bubble Powered by a Super PeVatron

We report the detection of a $\gamma$-ray bubble spanning at least 100$\rm deg^2$ in ultra high energy (UHE) up to a few PeV in the direction of the star-forming region Cygnus X, implying the presence Super PeVatron(s) accelerating protons to at least 10 PeV. A log-parabola form with the photon index $\Gamma (E) = (2.71 \pm 0.02) + (0.11 \pm 0.02) \times \log_{10} (E/10 \ {\rm TeV})$ is found fitting the gamma-ray energy spectrum of the bubble well. UHE sources, `hot spots' correlated with very massive molecular clouds, and a quasi-spherical amorphous $\gamma$-ray emitter with a sharp central brightening are observed in the bubble. In the core of $\sim 0.5^{\circ}$, spatially associating with a region containing massive OB association (Cygnus OB2) and a microquasar (Cygnus X-3), as well as previously reported multi-TeV sources, an enhanced concentration of UHE $\gamma$-rays are observed with 2 photons at energies above 1 PeV. The general feature of the bubble, the morphology and the energy spectrum, are reasonably reproduced by the assumption of a particle accelerator in the core, continuously injecting protons into the ambient medium.

==> authorlist20230423.tex <==
 
\author[1,2,3]{Zhen Cao}
\affiliation[1]{Key Laboratory of Particle Astrophyics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China}
\affiliation[2]{University of Chinese Academy of Sciences, 100049 Beijing, China}
\affiliation[3]{Tianfu Cosmic Ray Research Center, 610000 Chengdu, Sichuan,  China}
 
\author[4,5]{F. Aharonian}
\affiliation[4]{Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland }
\affiliation[5]{Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany}
 
\author[6,7]{Q. An}
\affiliation[6]{State Key Laboratory of Particle Detection and Electronics, China}
\affiliation[7]{University of Science and Technology of China, 230026 Hefei, Anhui, China}
 
\author[8]{Axikegu}
\affiliation[8]{School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China}
 
\author[1,3]{Y.X. Bai}

\author[9]{Y.W. Bao}
\affiliation[9]{School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China}
 
\author[10]{D. Bastieri}
\affiliation[10]{Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China}
 
\author[1,2,3]{X.J. Bi}

 
\author[1,3]{Y.J. Bi}

 
\author[10]{J.T. Cai}

 
\author[11]{Q. Cao}
\affiliation[11]{Hebei Normal University, 050024 Shijiazhuang, Hebei, China}
 
\author[7]{W.Y. Cao}
 
\author[6,7]{Zhe Cao}

 
\author[12]{J. Chang}
\affiliation[12]{Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China}
 
\author[1,3,6]{J.F. Chang}

 
\author[13]{A.M. Chen}
\affiliation[13]{Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China}
 
\author[1,2,3]{E.S. Chen}

 
\author[14]{Liang Chen}
\affiliation[14]{Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China}
 
\author[8]{Lin Chen}

 
\author[8]{Long Chen}
 
\author[1,3]{M.J. Chen}

 
\author[1,3,6]{M.L. Chen}

\author[8]{Q.H. Chen}

 
\author[1,2,3]{S.H. Chen}

 
\author[1,3]{S.Z. Chen}

 
\author[15]{T.L. Chen}
\affiliation[15]{Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China}
 
\author[9]{Y. Chen}
 
\author[1,3]{N. Cheng}

 
\author[1,3]{Y.D. Cheng}

 
\author[12]{M.Y. Cui}

 
\author[11]{S.W. Cui}

 
\author[16]{X.H. Cui}
\affiliation[16]{National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China}
 
\author[17]{Y.D. Cui}
\affiliation[17]{School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China}
 
\author[18]{B.Z. Dai}
\affiliation[18]{School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China}
 
\author[1,3,6]{H.L. Dai}

 
\author[7]{Z.G. Dai}
 
\author[15]{Danzengluobu}

 
\author[19]{D. della Volpe}
\affiliation[19]{D\'epartement de Physique Nucl\'eaire et Corpusculaire, Facult\'e de Sciences, Universit\'e de Gen\`eve, 24 Quai Ernest Ansermet, 1211 Geneva, Switzerland}
 
\author[1,2,3]{X.Q. Dong}

 
\author[12]{K.K. Duan}

 
\author[10]{J.H. Fan}
 
\author[12]{Y.Z. Fan}
 
\author[18]{J. Fang}
 
\author[1,3]{K. Fang}

 
\author[20]{C.F. Feng}
\affiliation[20]{Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China}
 
\author[12]{L. Feng}
 
\author[1,3]{S.H. Feng}
 
\author[20]{X.T. Feng}
 
\author[15]{Y.L. Feng}
 
\author[21]{S. Gabici}
\affiliation[21]{APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France}
 
\author[1,3]{B. Gao}
 
\author[20]{C.D. Gao}
 
\author[1,2,3]{L.Q. Gao}
 
\author[15]{Q. Gao}
 
\author[1,3]{W. Gao}
 
\author[1,2,3]{W.K. Gao}
 
\author[18]{M.M. Ge}
 
\author[1,3]{L.S. Geng}
 
\author[13]{G. Giacinti}
 
\author[22]{G.H. Gong}
\affiliation[22]{Department of Engineering Physics, Tsinghua University, 100084 Beijing, China}
 
\author[1,3]{Q.B. Gou}
 
\author[1,3,6]{M.H. Gu}
 
\author[14]{F.L. Guo}
 
\author[8]{X.L. Guo}
 
\author[1,3]{Y.Q. Guo}
 
\author[12]{Y.Y. Guo}
 
\author[23]{Y.A. Han}
\affiliation[23]{School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China}
 
\author[1,2,3]{H.H. He}
 
\author[12]{H.N. He}
 
\author[12]{J.Y. He}
 
\author[17]{X.B. He}
 
\author[8]{Y. He}
 
\author[19]{M. Heller}
 
\author[17]{Y.K. Hor}
 
\author[1,2,3]{B.W. Hou}

 
\author[1,3]{C. Hou}
 
\author[24]{X. Hou}
\affiliation[24]{Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China}
 
\author[1,2,3]{H.B. Hu}

 
\author[7,12]{Q. Hu}

 
\author[1,2,3]{S.C. Hu}

 
\author[8]{D.H. Huang}
 
\author[1,3]{T.Q. Huang}

 
\author[17]{W.J. Huang}
 
\author[20]{X.T. Huang}
 
\author[12]{X.Y. Huang}
 
\author[1,2,3]{Y. Huang}
 
\author[8]{Z.C. Huang}
 
\author[1,3,6]{X.L. Ji}
 
\author[8]{H.Y. Jia}
 
\author[20]{K. Jia}
 
\author[6,7]{K. Jiang}

 
\author[1,3]{X.W. Jiang}
 
\author[18]{Z.J. Jiang}
 
\author[8]{M. Jin}
 
\author[25]{M.M. Kang}
\affiliation[25]{College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China}
 
\author[1,3]{T. Ke}
 
\author[26]{D. Kuleshov}
\affiliation[26]{Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia}
 
\author[26,27]{K. Kurinov}
\affiliation[27]{Moscow Institute of Physics and Technology, 141700 Moscow, Russia}
 
\author[11]{B.B. Li}
 
\author[6,7]{Cheng Li}

 
\author[1,3]{Cong Li}

 
\author[1,2,3]{D. Li}

 
\author[1,3,6]{F. Li}

 
\author[1,3]{H.B. Li}

 
\author[1,3]{H.C. Li}

 
\author[7,12]{H.Y. Li}

 
\author[7,12]{J. Li}

 
\author[7]{Jian Li}
 
\author[1,3,6]{Jie Li}

 
\author[1,3]{K. Li}
 
\author[20]{W.L. Li}
 
\author[13]{W.L. Li}
 
\author[1,3]{X.R. Li}

 
\author[6,7]{Xin Li}

 
\author[1,2,3]{Y.Z. Li}

 
\author[1,3]{Zhe Li}
 
\author[28]{Zhuo Li}
\affiliation[28]{School of Physics, Peking University, 100871 Beijing, China}
 
\author[29]{E.W. Liang}
\affiliation[29]{School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China}
 
\author[29]{Y.F. Liang}
 
\author[17]{S.J. Lin}
 
\author[7]{B. Liu}
 
\author[1,3]{C. Liu}

 
\author[20]{D. Liu}
 
\author[8]{H. Liu}
 
\author[23]{H.D. Liu}
 
\author[1,3]{J. Liu}

 

 
\author[1,3]{J.Y. Liu}

 
\author[15]{M.Y. Liu}
 
\author[9]{R.Y. Liu}
 
\author[8]{S.M. Liu}
 
\author[1,3]{W. Liu}

 
\author[10]{Y. Liu}
 
\author[22]{Y.N. Liu}
 
\author[18]{R. Lu}
 
\author[17]{Q. Luo}
 
\author[1,3]{H.K. Lv}
 
\author[28]{B.Q. Ma}
 
\author[1,3]{L.L. Ma}

 
\author[1,3]{X.H. Ma}

 
\author[24]{J.R. Mao}
 
\author[1,3]{Z. Min}

 
\author[30]{W. Mitthumsiri}
\affiliation[30]{Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand}
 
\author[23]{H.J. Mu}
 
\author[1,3]{Y.C. Nan}
 
\author[21]{A. Neronov}
 
\author[17]{Z.W. Ou}
 
\author[8]{B.Y. Pang}
 
\author[30]{P. Pattarakijwanich}
 
\author[10]{Z.Y. Pei}
 
\author[1,3]{M.Y. Qi}

 
\author[11]{Y.Q. Qi}
 
\author[1,3]{B.Q. Qiao}

 
\author[7]{J.J. Qin}
 
\author[30]{D. Ruffolo}
 
\author[30]{A. S\'aiz}
 
\author[21]{D. Semikoz}
 
\author[17]{C.Y. Shao}
 
\author[11]{L. Shao}
 
\author[26,27]{O. Shchegolev}

 
\author[1,3]{X.D. Sheng}

 
\author[31]{F.W. Shu}
\affiliation[31]{Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology, Nanchang University, 330031 Nanchang, Jiangxi, China}
 
\author[28]{H.C. Song}
 
\author[26,27]{Yu.V. Stenkin}

 
\author[26]{V. Stepanov}
 
\author[12]{Y. Su}
 
\author[8]{Q.N. Sun}
 
\author[29]{X.N. Sun}
 
\author[32]{Z.B. Sun}
\affiliation[32]{National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China}
 
\author[17]{P.H.T. Tam}
 
\author[31]{Q.W. Tang}
 
\author[6,7]{Z.B. Tang}

 
\author[2,16]{W.W. Tian}

 
\author[32]{C. Wang}
 
\author[8]{C.B. Wang}
 
\author[7]{G.W. Wang}
 
\author[10]{H.G. Wang}
 
\author[17]{H.H. Wang}
 
\author[24]{J.C. Wang}
 
\author[9]{K. Wang}

\author[20]{L.P. Wang}
 
\author[1,3]{L.Y. Wang}

 
\author[8]{P.H. Wang}
 
\author[20]{R. Wang}
 
\author[17]{W. Wang}
 
\author[29]{X.G. Wang}
 
\author[9]{X.Y. Wang}
 
\author[8]{Y. Wang}
 
\author[1,3]{Y.D. Wang}
 
\author[1,3]{Y.J. Wang}

 
\author[25]{Z.H. Wang}
 
\author[18]{Z.X. Wang}
 
\author[13]{Zhen Wang}
 
\author[1,3,6]{Zheng Wang}

 
\author[12]{D.M. Wei}
 
\author[12]{J.J. Wei}
 
\author[1,2,3]{Y.J. Wei}
 
\author[18]{T. Wen}
 
\author[1,3]{C.Y. Wu}

 
\author[1,3]{H.R. Wu}

 
\author[1,3]{S. Wu}

 
\author[12]{X.F. Wu}
 
\author[7]{Y.S. Wu}
 
\author[1,3]{S.Q. Xi}

 
\author[7,12]{J. Xia}

 
\author[8]{J.J. Xia}
 
\author[2,14]{G.M. Xiang}

 
\author[11]{D.X. Xiao}
 
\author[1,3]{G. Xiao}

 
\author[1,3]{G.G. Xin}

 
\author[8]{Y.L. Xin}
 
\author[14]{Y. Xing}
 
\author[1,2,3]{Z. Xiong}

 
\author[13]{D.L. Xu}
 
\author[1,2,3]{R.F. Xu}

 
\author[28]{R.X. Xu}
 
\author[25]{W.L. Xu}
 
\author[20]{L. Xue}
 
\author[18]{D.H. Yan}
 
\author[12]{J.Z. Yan}
 
\author[1,3]{T. Yan}

 
\author[25]{C.W. Yang}
 
\author[11]{F. Yang}
 
\author[1,3,6]{F.F. Yang}

 
\author[17]{H.W. Yang}
 
\author[17]{J.Y. Yang}
 
\author[17]{L.L. Yang}
 
\author[1,3]{M.J. Yang}
 
\author[7]{R.Z. Yang}
 
\author[18]{S.B. Yang}
 
\author[25]{Y.H. Yao}
 
\author[1,3]{Z.G. Yao}

 
\author[22]{Y.M. Ye}
 
\author[1,3]{L.Q. Yin}

 
\author[20]{N. Yin}
 
\author[1,3]{X.H. You}

 
\author[1,2,3]{Z.Y. You}

 
\author[7]{Y.H. Yu}
 
\author[12]{Q. Yuan}
 
\author[1,2,3]{H. Yue}
 
\author[12]{H.D. Zeng}
 
\author[1,3,6]{T.X. Zeng}

 
\author[18]{W. Zeng}
 
\author[1,3]{M. Zha}

 
\author[9]{B.B. Zhang}
 
\author[8]{F. Zhang}
 
\author[9]{H.M. Zhang}
 
\author[1,3]{H.Y. Zhang}

 
\author[16]{J.L. Zhang}
 
\author[10]{L.X. Zhang}
 
\author[18]{Li Zhang}
 
\author[18]{P.F. Zhang}
 
\author[7,12]{P.P. Zhang}

 
\author[7,12]{R. Zhang}

 
\author[2,16]{S.B. Zhang}

 
\author[11]{S.R. Zhang}
 
\author[1,3]{S.S. Zhang}

 
\author[9]{X. Zhang}
 
\author[1,3]{X.P. Zhang}

 
\author[8]{Y.F. Zhang}
 
\author[1,12]{Yi Zhang}

 
\author[1,3]{Yong Zhang}

\author[8]{B. Zhao}
 
\author[1,3]{J. Zhao}

 
\author[6,7]{L. Zhao}

 
\author[11]{L.Z. Zhao}
 
\author[12,20]{S.P. Zhao}

 
\author[32]{F. Zheng}
 
\author[1,3]{B. Zhou}

 
\author[13]{H. Zhou}
 
\author[14]{J.N. Zhou}
 
\author[31]{M. Zhou}
 
\author[9]{P. Zhou}
 
\author[25]{R. Zhou}
 
\author[8]{X.X. Zhou}
 
\author[20]{C.G. Zhu}
 
\author[8]{F.R. Zhu}
 
\author[16]{H. Zhu}
 
\author[1,2,3,6]{K.J. Zhu}
 
\author[1,3]{X. Zuo}
%\collaboration{The LHAASO Collaboration}

